Validation of 3GPP TR 38.901 Indoor Hotspot Path Loss Model Based on Measurements Conducted at 6.75, 16.95, 28, and 73 GHz for 6G and Beyond

This paper presents a thorough validation of the Third Generation Partnership Project (3GPP) Technical Report (TR) 38.901 indoor hotspot (InH) path loss model, as part of the 3GPP Release 19 study on "Channel model validation of TR 38.901 for 7-24 GHz," for 6G standardization. Specifically, we validate the 3GPP TR 38.901 path loss model for the InH scenario in both line of sight (LOS) and non line of sight (NLOS) channel conditions, using the floating intercept (FI) and alpha-beta-gamma (ABG) path loss models. The validation focuses on specific frequencies, including 6.75 GHz and 16.95 GHz, as well as the broader 7-24 GHz and 0.5-100 GHz frequency ranges. The validation is based on real-world measurements conducted at 6.75 GHz, 16.95 GHz, 28 GHz, and 73 GHz by NYU WIRELESS using a 1 GHz wideband time domain based sliding correlation channel sounder in the InH scenario for both LOS and NLOS channel conditions. Our results confirm that the 3GPP TR 38.901 path loss model for the InH scenario remains valid for the 7-24 GHz range in both LOS and NLOS conditions and provide valuable input for 6G standardization efforts.

==> Sections/as.tex <==
\begin{figure}[t!]
    \centering
\includegraphics[width=9cm,height=10cm,keepaspectratio]{Figures/asa_6.75ghz_los_nlos_meas.eps}
    \caption{6.75 ghz ci model fit to meas data nd 3gpp (los/nlos option 1).}
    \vspace{-0.2in}
    \label{fig:indoor_snr}
\end{figure}


\begin{figure}[t!]
    \centering
\includegraphics[width=9cm,height=10cm,keepaspectratio]{Figures/asa_16.95ghz_los_nlos_meas.eps}
    \caption{6.75 ghz ci model fit to meas data nd 3gpp (los/nlos option 1).}
    \vspace{-0.2in}
    \label{fig:indoor_snr}
\end{figure}




% this paper has lgDS values and ecdf. 
\renewcommand{\arraystretch}{1.5}
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|p{2.5em}|c|r|r|r|r|}
  \hline
    \multirow{2}[4]{2em}{Freq. (GHz)} & \multirow{2}[4]{*}{Env.} & \multicolumn{2}{c|}{Measured (lgASA)} & \multicolumn{2}{c|}{3GPP (lgASA)} \\
\cline{3-6}          &       & \multicolumn{1}{c|}{$\mu$} & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c|}{$\mu$} & \multicolumn{1}{c|}{$\sigma$} \\
   \hline
    \multirow{2}[4]{*}{6.75} & LOS   & 1.8 & 0.1  & 1.6  & 0.2 \\
\cline{2-6}          & NLOS  & 1.8 & 0.1   & 1.8 & 0.2 \\
   \hline
    \multirow{2}[4]{*}{16.95} & LOS   & 1.2 & 0.7  & 1.5  & 0.3 \\
\cline{2-6}          & NLOS  & 1.5 & 0.5  & 1.7 & 0.2 \\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
